Radial velocities of narrow emission line components in the spectra of T Tauri stars

We studied rotational modulation of the radial velocities of narrow emission lines in four classical T Tauri stars. We found that the previously declared shift of the mean velocity of neutral and ionized helium lines relative to the mean radial velocity of the star is not associated with the inflow of accreted gas into the hotspot, since the radial velocity curves for lines with different velocity shifts should exhibit phase shifts relative to each other, while the observed phase shifts are absent within their uncertainties and do not correspond to the observed line velocity shifts. This means that the line shifts are not caused by the actual gas motion. For neutral helium lines, the shifts can be explained by the large optical thickness of the lines and the Stark effect at plasma parameters expected at the base of the accretion column of T Tauri stars.

==> journals.tex <==
\newcommand{\aj}{Astronomical Journal}
\newcommand{\actaa}{Acta Astronomica}
\newcommand{\araa}{Annual Review of Astron and Astrophys}
\newcommand{\apj}{Astrophysical Journal}
\newcommand{\apjl}{Astrophysical Journal, Letters}
\newcommand{\apjs}{Astrophysical Journal, Supplement}
\newcommand{\ao}{Applied Optics}
\newcommand{\apss}{Astrophysics and Space Science}
\newcommand{\aap}{Astronomy and Astrophysics}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}
\newcommand{\aaps}{Astronomy and Astrophysics, Supplement}
\newcommand{\azh}{Astronomicheskii Zhurnal}
\newcommand{\baas}{Bulletin of the AAS}
\newcommand{\caa}{Chinese Astronomy and Astrophysics}
\newcommand{\cjaa}{Chinese Journal of Astronomy and Astrophysics}
\newcommand{\icarus}{Icarus}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\jrasc}{Journal of the RAS of Canada}
\newcommand{\memras}{Memoirs of the RAS}
\newcommand{\mnras}{Monthly Notices of the RAS}
\newcommand{\na}{New Astronomy}
\newcommand{\nar}{New Astronomy Review}
\newcommand{\pra}{Physical Review A: General Physics}
\newcommand{\prb}{Physical Review B: Solid State}
\newcommand{\prc}{Physical Review C}
\newcommand{\prd}{Physical Review D}
\newcommand{\pre}{Physical Review E}
\newcommand{\prl}{Physical Review Letters}
\newcommand{\pasa}{Publications of the Astron. Soc. of Australia}
\newcommand{\pasp}{Publications of the ASP}
\newcommand{\pasj}{Publications of the ASJ}
\newcommand{\rmxaa}{Revista Mexicana de Astronomia y Astrofisica}
\newcommand{\qjras}{Quarterly Journal of the RAS}
\newcommand{\skytel}{Sky and Telescope}
\newcommand{\solphys}{Solar Physics}
\newcommand{\sovast}{Soviet Astronomy}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\zap}{Zeitschrift fuer Astrophysik}
\newcommand{\nat}{Nature}
\newcommand{\iaucirc}{IAU Cirulars}
\newcommand{\aplett}{Astrophysics Letters}
\newcommand{\apspr}{Astrophysics Space Physics Research}
\newcommand{\bain}{Bulletin Astronomical Institute of the Netherlands}
\newcommand{\fcp}{Fundamental Cosmic Physics}
\newcommand{\gca}{Geochimica Cosmochimica Acta}
\newcommand{\grl}{Geophysics Research Letters}
\newcommand{\jcp}{Journal of Chemical Physics}
\newcommand{\jgr}{Journal of Geophysics Research}
\newcommand{\jqsrt}{Journal of Quantitiative Spectroscopy and Radiative Transfer}
\newcommand{\memsai}{Mem. Societa Astronomica Italiana}
\newcommand{\nphysa}{Nuclear Physics A}
\newcommand{\physrep}{Physics Reports}
\newcommand{\physscr}{Physica Scripta}
\newcommand{\planss}{Planetary Space Science}
\newcommand{\procspie}{Proceedings of the SPIE}

